Assuming Just Enough Fairness to make Session Types Complete for Lock-freedom

We investigate how different fairness assumptions affect results concerning lock-freedom, a typical liveness property targeted by session type systems. We fix a minimal session calculus and systematically take into account all known fairness assumptions, thereby identifying precisely three interesting and semantically distinct notions of lock-freedom, all of which having a sound session type system. We then show that, by using a general merge operator in an otherwise standard approach to global session types, we obtain a session type system complete for the strongest amongst those notions of lock-freedom, which assumes only justness of execution paths, a minimal fairness assumption for concurrent systems.

==> appD.tex <==
% !TEX root = main.tex
\subsection{Notions of lock-freedom for our reactive semantics}\label{app:D}
\commP{not yet checked}

\comP{currently stuff copied from Sect IIE -- needs to be polished, 
and combined with App E}

We conclude with a classification taking into account all liveness properties we have considered,
including those \rpR{arrising}{arising } from the reactive semantics.


\begin{proposition}{create label}
If $\pi$ is an \F-fair path according to the semantics of Figure~\ref{fig:red},
then $\pi$ is also an  \F-fair path according to Figure~\ref{fig:reactive}.
\end{proposition}
\comP{proof to be provided; should shorten the proof of Prop 4 (I hope) -- only for the presented fairness notions}

\begin{proposition}{inclusion appD}
$\N\models\Live{\F} \Rightarrow \N\models \React{\F}$,
for any fairness assumption $\F$ and network $\N$.
\end{proposition}
\comH{Does this proof only work for properties stronger than $\J$? What about $\W\T$?}
\comP{I believe, the proof does hold for justness as well, but needs a slightly different argument; 
if a location $p$ is involved in a $\tau$-step stemming from choice or recursion, 
$p$ will be involved in a communication later on.}
\comP{Although I did not construct a counter-example, I think 
the lemma only works for guarded networks}
\commH{I was worried that there might be provisos that mean we need to stick to the notions of weak/strong fairness provided rather than all notions of fairness.}
\begin{proof}
Every $\F$-fair path $\pi$ according to Figure~\ref{fig:reactive}
maps to some $\F$-fair path $\hat{\pi}$ according to Figure~\ref{fig:red}, by adding finitely many $\tau$-transitions before each communication \chP{and recursion}.
Hence, since, for this session calculus, there is a bound on the number of $\tau$-transitions \commP{we calculate on a finite-state system} 
before every interaction transition, if infinitely many transitions involving a component on $\hat{\pi}$, then there are infinitely many transitions involving the same component in $\pi$.

Trivially, if a component successfully terminates on $\hat{\pi}$ it must also terminate on $\pi$.
Now, for every $\F$-fair path $\pi$ of $\N$ according to Figure~\ref{fig:reactive}, hence, assuming network $\N$ is $\Live{\F}$, every component either successfully terminates or acts infinitely often on $\hat{\pi}$ and hence also does so on $\pi$.
\end{proof}
\chP\hrule\commP{jumping to Sect III for the moment}
Further to the above inclusion, some notions of fairness that collapse in the classification in Figure~\ref{reduced taxonomy} become distinguished for a reactive semantics.
The most important distinction for our arguments in this paper is that $\React{\J}$ is strictly stronger than $\React{\W\C}$ (but remains stronger than $\React{\St\C}$); that is, the counterpart of Proposition~\ref{pr:WC} does not hold in the reactive setting, as demonstrated by the following example.
\begin{example}{reactive:early AppD}
The following network satisfies $\React{\W\C}$ (and hence also $\React{\St\C}$), but does not satisfy $\Live{\St\C}$ (and hence also does not satisfy $\Live{J}$).
\[
\begin{array}[t]{rl}
&
\buyer\mbox{\Large\textlbrackdbl}
 \rec{X} \big(
  \begin{array}[t]{l}
  \send{\seller1}{\order1} ; X
  \\
  \oplus ~
  \send{\seller2}{\order2}; \send{\seller1}{\done}~\big)~\mbox{\Large\textrbrackdbl}
  \end{array}
\\
\pipar
&
\loc{\seller1}{
 \rec{Y} \big(
  \recv{\buyer}{\order1} ;  Y
  +
  \recv{\buyer}{\done} 
  ~\big)
}
\\
\pipar
&
\loc{\seller2}{
 \recv{\buyer}{\order2}
}
\end{array}
\]
The above example does not satisfy $\Live{\St\C}$, since, due to the $\tau$ transition solving internal choice in Figure~\ref{fig:red}, there is an $\St\C$-path where the $\buyer$ never commits to communicating with $\seller2$.
But there is no such $\W\C$-path according to Figure~\ref{fig:reactive}, since a transition stemming from $\seller2$ is perpetually enabled on all $\W\C$-paths, when appealing to Figure~\ref{fig:reactive}.
\end{example}
The above example also shows that $\React{\SC}$ is strictly weaker than $\Live{\SC}$.
However, $\React{\SC}$ remains strictly weaker than $\React{\St\T}$ since Example~\ref{ex:binaryext:early} does not satisfy $\React{\SC}$.\footnote{
We clarify that in~\cite{Severi2019} (Example 2.14) there is a remark, to the effect that our Example~\ref{ex:binaryext:early} satisfies $\React{\SC}$, since they use a reactive semantics and cite Kobayashi~\cite{Kobayashi2002} for a notion of fairness. Under this reading that remark is incorrect; however we believe their intention is to say that Example~\ref{ex:binaryext:early} satisfies $\React{\St\T}$, which is correct.
}

Another distinction made by a reactive semantics is that, $\React{\Pr}$ is strictly stronger than $\React{\W\T}$, and, furthermore, $\React{\W\T}$ 
is unrelated to $\React{\St\C}$ and $\React{\J}$.
To see this separation, observe that Example~\ref{ex:sc-j:early} satisfies $\React{\W\T}$ but not $\React{\SC}$ (hence neither $\React{\J}$ nor $\React{P}$); while in the other direction Example~\ref{ex:jt-j}, below, satisfies $\React{\J}$ (hence also $\React{\SC}$), but not $\React{\W\T}$.
\begin{example}{jt-j}
The following example shows that $\React{\W\T}$ is not stronger than $\React{\J}$.
\begin{array}[t]{rl}
&
\loc{\trader1}{
 \rec{X}
  \send{\trader2}{\order}; \recv{\trader2}{\order}; X
}
\\
\pipar
&
\loc{\trader2}{
 \rec{Y}
  \recv{\trader1}{\order} ;   \send{\trader1}{\order} ;  Y
}
\\
\pipar
&
\loc{\accountant}{
 \send{\auditor}{\report}
}
\\
\pipar
&
\loc{\auditor}{
 \recv{\accountant}{\report} 
}
\end{array}
\end{example}
The above network satisfies $\React{\J}$, since both pairs of interacting components are concurrent to each other hence communicate infinitely often or successfully terminate on every $\J$-path.
To see why Example~\ref{ex:jt-j} does not satisfy $\React{\W\T}$, observe that the transition in which the report is exchanged changes after each step and hence no transition is perpetually enabled; and there are $\W\T$-paths where a pair of components does not act infinitely often or successfully terminate.

A critical observation in our argument for $\J$ is that, despite divergences for many notions of fairness, lock-freedom remains constant for $\J$ regardless of the choice of semantics for our session calculus. That is $\Live{\J}$ and $\React{\J}$ coincide.
\begin{proposition}{J AppD}
A network satisfies $\React{\J}$ iff it satisfies $\Live{\J}$.
\end{proposition}
\begin{proof}
\comH{Proof sketch.}
By Proposition~\ref{pr:inclusion}, it remains to prove the only ``if'' direction.
It is sufficient to observe that every $\J$-path $\pi$ according to Figure~\ref{fig:red} maps to some $\J$-path $\pi'$ according to Figure~\ref{fig:reactive} by removing $\tau$-transitions, since if a $\tau$-transition $t$ is enabled in some state, leading to some $\comm{p}{\lambda}{q}$-transition, then another $\tau$-transition $u$ must occur afterwards such that $t \not\conc u$, which makes some $\comm{p'}{\lambda'}{q'}$-transition inevitable. The corresponding $\comm{p'}{\lambda'}{q'}$ transition in $\pi'$, say $t'$ is such that $t' \not\conc u'$, where $u'$ is the $\comm{p}{\lambda}{q}$-transition in $\pi'$ corresponding to $t$.
\end{proof}

The above proposition suggests that $\J$ is a more robust notion that $\W\C$, and, indeed, we will see that our completeness results are robust for all choices of semantics only if we assume $\J$.
We highlight later in this paper, at the appropriate points in Observation~\ref{obs:WC complete}
and Observation~\ref{obs:reactive race},
the consequences of collapses that hold for the semantics with $\tau$-transitions, but not the reactive semantics.





\begin{figure}
\input{latticefull}
\centerline{\raisebox{-5ex}{\box\graph}}
\caption{Classification incorporating reactive notions of lock freedom and indicating the relationships with guarded well-typedness.}
\label{reactive taxonomy Appendix}
\end{figure}


Regarding reactive semantics, further to distinction mentioned in Section~\ref{sec:reactive} the counterpart of Proposition~\ref{pr:SA=P live} does not hold, since Example~\ref{ex:binaryext:early} is $\React{\W\A}$ and hence $\React{\St\A}$ but not $\React{\J}$ and hence not $\React{\Pr}$ or $\Live{\W\A}$. Notice, since Example~\ref{ex:binaryext:early} is not guardedly well-typed, our session type system cannot be complete for $\React{\W\A}$, strengthening further our claim that $\J$ is the appropriate choice of fairness assumption for our session type system. Furthermore, the following example separates $\React{\W\A}$ from $\React{\St\A}$.
\begin{example}{WA}
The following variant of Example~\ref{ex:binaryext:early} satisfies $\React{\St\A}$, but does not satisfy $\React{\W\A}$, or $\Live{\St\C}$.
\[
\begin{array}{rl}
&
\loc{q}{ \rec{X}\left( \send{q}{a}; \send{q}{d} ; X \oplus \send{q}{b} ; X \right) }
\\ \pipar &
\loc{q}{ \rec{Y}\left( \recv{p}{a} ; \recv{q}{d} ; Y + \recv{p}{b} ; \send{r}{c} ; Y \right) } 
\\ \pipar &
\loc{r}{ \rec{Z}\left( \recv{q}{c} ; Z \right) }
\end{array}
\]
The above network is also not guardedly \welltyped. 
\end{example}

To distinguish $\React{\St\A}$ from $\React{\St\T}$ we require an example with a race due to non-determinism of such as in the following examples.
\begin{example}{noo-determinism}
The following is $\Live{\St\T}$ and hence also $\React{\St\T}$.
It does not however satisfy $\React{\St\A}$ or $\React{\W\T}$.
\[
\begin{array}{rl}
&
\loc{p}{ \rec{X} \left( \send{q}{d} ; \left( \send{q}{a};  X \oplus \send{q}{a} ; X \right) \right) }
\\ \pipar &
\loc{q}{ \rec{Y}  \recv{p}{d} ; \left( \recv{p}{a} ; Y + \recv{p}{a} ; \send{r}{c} ; Y \right) } 
\\ \pipar &
\loc{r}{ \rec{Z}\left( \recv{q}{c} ; Z \right) }
\end{array}
\]
Similarly, the following network satisfies $\React{\W\T}$ but does not satisfy $\React{\St\A}$.
\[
\begin{array}{rl}
&
\loc{p}{ \rec{X}\left( \send{q}{a} ; X + \send{q}{a} ; \send{r}{c} ; X\right) }
\\ \pipar &
\loc{q}{ \rec{Y}\left( \recv{p}{a} ; Y \right) } 
\\ \pipar &
\loc{r}{ \rec{Z}\left( \recv{p}{c} ; Z \right) }
\end{array}
\]
\end{example}

The complexity of the resulting classification in Figure~\ref{reactive taxonomy Appendix} and the absence of any new completeness result stemming from these notions of lock freedom helps explain why we do not emphasise the reactive semantics in the body of this paper.
The sole completenss result that holds is the one indicated concerning $\Live{\J}$.





==> latticeR.tex <==
\expandafter\ifx\csname graph\endcsname\relax
   \csname newbox\expandafter\endcsname\csname graph\endcsname
\fi
\ifx\graphtemp\undefined
  \csname newdimen\endcsname\graphtemp
\fi
\expandafter\setbox\csname graph\endcsname
 =\vtop{\vskip 0pt\hbox{%
    \graphtemp=.5ex
    \advance\graphtemp by 2.381in
    \rlap{\kern 0.000in\lower\graphtemp\hbox to 0pt{\hss $\Live{\textrm{P}} = \React{\textrm{P}}$\hss}}%
    \graphtemp=.5ex
    \advance\graphtemp by 1.905in
    \rlap{\kern 0.000in\lower\graphtemp\hbox to 0pt{\hss $\Live{\textrm{J}} = \React{\textrm{J}}$\hss}}%
    \graphtemp=.5ex
    \advance\graphtemp by 1.429in
    \rlap{\kern 0.000in\lower\graphtemp\hbox to 0pt{\hss $\Live{\textrm{SC}}$\hss}}%
    \graphtemp=.5ex
    \advance\graphtemp by 1.429in
    \rlap{\kern 0.714in\lower\graphtemp\hbox to 0pt{\hss $\React{\textrm{WC}}$\hss}}%
    \graphtemp=.5ex
    \advance\graphtemp by 0.952in
    \rlap{\kern 0.000in\lower\graphtemp\hbox to 0pt{\hss $\React{\textrm{SC}}$\hss}}%
    \graphtemp=.5ex
    \advance\graphtemp by 1.429in
    \rlap{\kern 1.429in\lower\graphtemp\hbox to 0pt{\hss $\React{\textrm{WT}}$\hss}}%
    \graphtemp=.5ex
    \advance\graphtemp by 0.476in
    \rlap{\kern 0.000in\lower\graphtemp\hbox to 0pt{\hss $\Live{\textrm{ST}} = \React{\textrm{ST}}$\hss}}%
    \graphtemp=.5ex
    \advance\graphtemp by 0.000in
    \rlap{\kern 0.000in\lower\graphtemp\hbox to 0pt{\hss \textit{deadlock-free}\hss}}%
\pdfliteral{
q [] 0 d 1 J 1 j
0.576 w
0.576 w
-1.728 -153 m
0 -145.8 l
S
1.8 -153 m
0 -145.8 l
S
0 -162.864 m
0 -145.8 l
S
12.24 -44.568 m
7.2 -39.096 l
S
14.256 -41.616 m
7.2 -39.096 l
S
95.76 -98.136 m
7.2 -39.096 l
S
-1.728 -50.184 m
0 -42.984 l
S
1.8 -50.184 m
0 -42.984 l
S
0 -59.976 m
0 -42.984 l
S
88.632 -110.16 m
95.616 -107.712 l
S
90.648 -113.184 m
95.616 -107.712 l
S
7.128 -166.68 m
95.616 -107.712 l
S
-1.728 -118.728 m
0 -111.528 l
S
1.8 -118.728 m
0 -111.528 l
S
0 -128.592 m
0 -111.528 l
S
37.224 -110.16 m
44.208 -107.712 l
S
39.24 -113.184 m
44.208 -107.712 l
S
7.128 -132.408 m
44.208 -107.712 l
S
12.24 -78.912 m
7.2 -73.368 l
S
14.256 -75.888 m
7.2 -73.368 l
S
44.28 -98.136 m
7.2 -73.368 l
S
-1.728 -15.912 m
0 -8.712 l
S
1.8 -15.912 m
0 -8.712 l
S
0 -25.704 m
0 -8.712 l
S
-1.728 -84.456 m
0 -77.256 l
S
1.8 -84.456 m
0 -77.256 l
S
0 -94.32 m
0 -77.256 l
S
Q
}%
    \hbox{\vrule depth2.381in width0pt height 0pt}%
    \kern 1.429in
  }%
}%


==> latticefull.tex <==
\expandafter\ifx\csname graph\endcsname\relax
   \csname newbox\expandafter\endcsname\csname graph\endcsname
\fi
\ifx\graphtemp\undefined
  \csname newdimen\endcsname\graphtemp
\fi
\expandafter\setbox\csname graph\endcsname
 =\vtop{\vskip 0pt\hbox{%
    \graphtemp=.5ex
    \advance\graphtemp by 2.857in
    \rlap{\kern 0.952in\lower\graphtemp\hbox to 0pt{\hss $\Live{\textrm{P}} = \Live{\textrm{SA}}  = \Live{\textrm{WA}} = \React{\textrm{P}}$\hss}}%
    \graphtemp=.5ex
    \advance\graphtemp by 2.381in
    \rlap{\kern 0.952in\lower\graphtemp\hbox to 0pt{\hss $\Live{\textrm{J}} = \React{\textrm{J}}$\hss}}%
    \graphtemp=.5ex
    \advance\graphtemp by 1.667in
    \rlap{\kern 0.000in\lower\graphtemp\hbox to 0pt{\hss \textit{guardedly typed}\hss}}%
    \graphtemp=.5ex
    \advance\graphtemp by 1.905in
    \rlap{\kern 0.952in\lower\graphtemp\hbox to 0pt{\hss $\Live{\textrm{SC}}$\hss}}%
    \graphtemp=.5ex
    \advance\graphtemp by 1.905in
    \rlap{\kern 1.667in\lower\graphtemp\hbox to 0pt{\hss $\React{\textrm{WC}}$\hss}}%
    \graphtemp=.5ex
    \advance\graphtemp by 1.429in
    \rlap{\kern 0.952in\lower\graphtemp\hbox to 0pt{\hss $\React{\textrm{SC}}$\hss}}%
    \graphtemp=.5ex
    \advance\graphtemp by 1.429in
    \rlap{\kern 1.667in\lower\graphtemp\hbox to 0pt{\hss $\React{\textrm{WA}}$\hss}}%
    \graphtemp=.5ex
    \advance\graphtemp by 1.667in
    \rlap{\kern 2.381in\lower\graphtemp\hbox to 0pt{\hss $\React{\textrm{WT}}$\hss}}%
    \graphtemp=.5ex
    \advance\graphtemp by 0.952in
    \rlap{\kern 0.952in\lower\graphtemp\hbox to 0pt{\hss $\React{\textrm{SA}}$\hss}}%
    \graphtemp=.5ex
    \advance\graphtemp by 0.476in
    \rlap{\kern 0.952in\lower\graphtemp\hbox to 0pt{\hss $\Live{\textrm{ST}} = \React{\textrm{ST}}$\hss}}%
    \graphtemp=.5ex
    \advance\graphtemp by 0.000in
    \rlap{\kern 0.952in\lower\graphtemp\hbox to 0pt{\hss \textit{deadlock-free}\hss}}%
\pdfliteral{
q [] 0 d 1 J 1 j
0.576 w
0.576 w
66.744 -187.344 m
68.544 -180.144 l
S
70.344 -187.344 m
68.544 -180.144 l
S
68.544 -197.136 m
68.544 -180.144 l
S
79.632 -45.864 m
75.24 -39.816 l
S
81.936 -43.056 m
75.24 -39.816 l
S
164.808 -114.48 m
75.24 -39.816 l
S
158.04 -128.808 m
164.736 -125.568 l
S
160.344 -131.544 m
164.736 -125.568 l
S
75.168 -200.232 m
164.736 -125.568 l
S
11.664 -130.968 m
6.984 -125.208 l
S
13.824 -128.088 m
6.984 -125.208 l
S
61.704 -166.32 m
6.984 -125.208 l
S
66.744 -153 m
68.544 -145.8 l
S
70.344 -153 m
68.544 -145.8 l
S
68.544 -162.864 m
68.544 -145.8 l
S
105.768 -144.432 m
112.752 -141.984 l
S
107.784 -147.456 m
112.752 -141.984 l
S
75.672 -166.68 m
112.752 -141.984 l
S
80.784 -113.184 m
75.816 -107.712 l
S
82.8 -110.16 m
75.816 -107.712 l
S
112.896 -132.408 m
75.816 -107.712 l
S
80.784 -78.912 m
75.816 -73.368 l
S
82.8 -75.888 m
75.816 -73.368 l
S
112.896 -98.136 m
75.816 -73.368 l
S
118.224 -118.728 m
120.024 -111.528 l
S
121.824 -118.728 m
120.024 -111.528 l
S
120.024 -128.592 m
120.024 -111.528 l
S
66.744 -15.912 m
68.544 -8.712 l
S
70.344 -15.912 m
68.544 -8.712 l
S
68.544 -25.704 m
68.544 -8.712 l
S
66.744 -84.456 m
68.544 -77.256 l
S
70.344 -84.456 m
68.544 -77.256 l
S
68.544 -94.32 m
68.544 -77.256 l
S
66.744 -50.184 m
68.544 -42.984 l
S
70.344 -50.184 m
68.544 -42.984 l
S
68.544 -59.976 m
68.544 -42.984 l
S
66.744 -118.728 m
68.544 -111.528 l
S
70.344 -118.728 m
68.544 -111.528 l
S
68.544 -128.592 m
68.544 -111.528 l
S
Q
}%
    \hbox{\vrule depth2.857in width0pt height 0pt}%
    \kern 2.381in
  }%
}%

